Learning MDPs from Features: Predict-Then-Optimize for Sequential Decision Problems by Reinforcement Learning

In the predict-then-optimize framework, the objective is to train a predictive model, mapping from environment features to parameters of an optimization problem, which maximizes decision quality when the optimization is subsequently solved. Recent work on decision-focused learning shows that embedding the optimization problem in the training pipeline can improve decision quality and help generalize better to unseen tasks compared to relying on an intermediate loss function for evaluating prediction quality. We study the predict-then-optimize framework in the context of sequential decision problems (formulated as MDPs) that are solved via reinforcement learning. In particular, we are given environment features and a set of trajectories from training MDPs, which we use to train a predictive model that generalizes to unseen test MDPs without trajectories. Two significant computational challenges arise in applying decision-focused learning to MDPs: (i) large state and action spaces make it infeasible for existing techniques to differentiate through MDP problems, and (ii) the high-dimensional policy space, as parameterized by a neural network, makes differentiating through a policy expensive. We resolve the first challenge by sampling provably unbiased derivatives to approximate and differentiate through optimality conditions, and the second challenge by using a low-rank approximation to the high-dimensional sample-based derivatives. We implement both Bellman--based and policy gradient--based decision-focused learning on three different MDP problems with missing parameters, and show that decision-focused learning performs better in generalization to unseen tasks.

==> challenge.tex <==
\section{Challenges}

\subsection{Simulator}
In the above setting, we assume our RL algorithm has unlimited accesses to the simulator. However, simulator might not always be available.

\paragraph{Solution}
One way to resolve the simulator issue is to leverage the past trajectories. We can build a simulator based on the past observation, where the more the new state action pair deviates from the past trajectories, the more penalty we get from using that state action pair.

\paragraph{Potential Issues}
If the past observation is sparse, very likely all the trajectories are disjoint. This will force the simulator we build based on past trajectories to incline just using the past trajectories. If we want to use the past trajectories to construct our simulator, we might want all the state action pairs to be relatively dense.

{\color{red} Any references on using past trajectories to build the simulator?}

\subsection{Counterfactual Regret and The Lack of Fully Specified Ground Truth}
This issue is due to the fact that our data might not contain the full description of the ground truth parameters (immediate rewards). For example, the past trajectories might contain where the rangers went and what they found along the trajectory. But we know nothing outside the trajectory. The ground truth only contains the necessary information in the trajectory. This creates an issue of measuring counterfactual regret, where we might want to try different trajectories in the past to see how good they are.

\paragraph{Solution}
I do not have a good solution to this yet. We could possibly use a similar idea of using other past trajectories to estimate what might have happened if a different strategy was chosen.


\subsection{Inaccurate Policy Gradient Estimate}
Although the gradient we get from the policy gradient theorem is unbiased, it is not the exact gradient that we are hoping to get. Similarly, the policy Hessian is also an unbiased estimate Hessian matrix only. But the product of two unbiased estimates is no longer an unbiased estimate (plus we need to do matrix inversion).

\paragraph{Solution (potential theorem from here)}
We can show how much deviation would the product of two unbiased estimates create.

\paragraph{Reference}
The study by Shen et al. \cite{shen2019hessian} about Hessian aided policy gradient.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please refer to Appendix~\ref{sec:challenges}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{Please refer to Appendix~\ref{sec:missing-proofs}}
\end{enumerate}
\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please refer to the supplementary material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please refer to Appendix~\ref{sec:experiment-setup}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to Appendix~\ref{sec:computing-infrastructure}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All data are synthetic except for the transition probabilities used to generate synthetic patients are taken from~\cite{killian2019learning}, and we provide reference to the papers that inspired them.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> legacy.tex <==

\begin{table}[t]
\caption{OPE performances of different methods on the test MDPs averaged over $30$ independent runs.
Decision-focused learning methods consistently outperform two-stage approach, with some exception using identity matrix based Hessian approximation which may lead to high gradient variance.
}\label{table:ope-trajectories}
\vspace{2mm}
\small
\centering
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{Snare} & \multicolumn{2}{c}{Tuberculosis} \\  \cmidrule(lr{.75em}){2-3} \cmidrule(lr{.75em}){4-5}
Trajectories         & Random                 & Near-optimal          & Random                   & Near-optimal  \\ \midrule
TS                  & $\cellcolor{lightred} 0.8 \! \pm \! 0.3 $  & $\cellcolor{lightred} 3.7 \! \pm \! 0.3 $ & $ \cellcolor{lightred} 35.8 \! \pm \! 1.5 $ & $\cellcolor{lightred} 38.7 \! \pm \! 1.6$ \\
% PG-Full             & $ -11.4 \! \pm \! 1.2 $ & $ 5.6 \! \pm \! 0.8 $ & N/A                    &  N/A                  & N/A                      & N/A \\ \hline
PG-W                & $ 1.2 \! \pm \! 0.4 $  & $ \cellcolor{lightgreen} 4.8 \! \pm \! 0.3 $ & $\cellcolor{lightgreen} 38.4 \! \pm \! 1.5$ & $40.8 \! \pm \! 1.7$ \\
% DF-B-Full        & $ -11.3 \! \pm \! 1.3 $ & $ \boldsymbol{15.7 \! \pm \! 1.3} $ & N/A                      & N/A                      & N/A & N/A \\ \hline
Bellman-W           & $ \cellcolor{lightgreen} 1.5 \! \pm \! 0.4 $  & $ 4.3 \! \pm \! 0.3 $ & $38.6 \! \pm \! 1.6$ & $\cellcolor{lightgreen} 41.1 \! \pm \! 1.7$ \\ \bottomrule
\end{tabular}
\end{table}
